Coherent gluon radiation: beyond leading-log accuracy

Results are presented for the medium-induced, soft coherent radiation spectrum for all $2\to 2$ partonic channels in QCD, at leading-order in $\alpha_s$ but beyond leading logarithmic accuracy. The general formula is valid in the full kinematic range of the underlying process, and reduces to previous results in special cases. The soft gluon radiation spectrum is expressed in terms of the color density matrix specific to each channel, quantifying the entanglement between the color components of the $2 \to 2$ production amplitude. Beyond the leading logarithm, the spectrum depends explicitly on the off-diagonal elements of this matrix, owing to the soft gluon's ability to probe the internal color structure of the parton pair.

==> macro.tex <==
%% DEFINITIONS  %%

\def\bc{\begin{center}}
\def\ec{\end{center}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bt{\begin{tabular}}
\def\et{\end{tabular}}
\def\ba{\begin{array}}
\def\ea{\end{array}}

\newcommand{\figscale}{1.0}  

\newcommand{\nn}{\nonumber} 
\newcommand{\ie}{{i.e.}}  
\newcommand{\eg}{{e.g.}}
\newcommand{\diag}{{\rm diag}}

\def\wv#1{\widetilde{#1}} 
\newcommand{\lqcd}{\Lambda_{_{\rm QCD}}}
\def\xtwo{x_{_2}}
\def\sun{{\rm SU}(\Nc)}
\newcommand{\as}{\al_s}
\newcommand{\unit}{{\mathds{1}}} 
\newcommand{\Nc}{\ensuremath{N}\xspace}
\newcommand{\CF}{C_F}
\newcommand{\xibar}{{\bar{\xi}}} 
\newcommand{\np}{n} 
\newcommand{\ns}{{\tilde n}} 

\newcommand{\morder}[1]{{\cal O}\left(#1 \right)}
\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\com}[2]{\left[{#1},{#2}\right]}
\newcommand{\ave}[1]{\langle{#1}\rangle}

\newcommand{\tf}{t_{\mathrm{f}}}
\newcommand{\R}{\textnormal{R}}
\newcommand{\Kvec}{{\boldsymbol K}}
\newcommand{\qvec}{{\boldsymbol q}}
\newcommand{\ella}{L_{_{\rm A}}}

\newcommand{\al}{\alpha}
\newcommand{\ga}{\gamma}
\newcommand{\all}{{\alpha, \lambda}}
\newcommand{\ball}{{\beta, \lambda}}
\newcommand{\gall}{{\ga, \lambda}}

\newcommand{\jpsi}{J/\psi}
\newcommand{\mt}{m_{_\perp}}
\newcommand{\pt}{p_{_\perp}}
\newcommand{\pp}{\ensuremath{\text{pp}}\xspace}
\newcommand{\pA}{\ensuremath{\text{pA}}\xspace}
\newcommand{\pPb}{\ensuremath{\text{pPb}}\xspace}
\newcommand{\pN}{p--N}
\newcommand{\dd}{{\rm d}}
\newcommand{\pd}{\partial}
\newcommand{\lsim}{\lesssim} 
\newcommand{\gsim}{\gtrsim}

\def\bm#1{\mbox{\boldmath$#1$}}
\newcommand{\Tr}{\mathrm{Tr}\,}
\newcommand{\tr}{\mathrm{tr}\,}
\newcommand{\trc}{\tr_{_{\! \! \rm c}}}
\newcommand{\trd}{\tr_{_{\! \! \rm d}}}
\newcommand{\tri}{\tr_{_{\! \! \rm irreps}}}
\newcommand{\trphi}{\tr_{_{\! \! \Phi}}}

\def\sighat{\hat{\sigma}}
\newcommand{\F}{{\cal F}}
\newcommand{\T}{\Theta}
\newcommand{\B}{\mathds{B}}
\newcommand{\Bbar}{\overline{\mathds{B}}}
\newcommand{\Bp}{{\cal B}_+}
\newcommand{\Bm}{{\cal B}_-}
\newcommand{\ADM}{{\cal Q}}
\newcommand{\Phat}{\hat{{\cal P}}}
\def\qhat{\hat{q}}
\newcommand{\dilog}{{\rm Li}_2}

\newcommand{\ket}[1]{\vert{#1}\rangle}
\newcommand{\bra}[1]{\langle{#1}\vert}
\newcommand{\tran}{^\intercal}

%%%%%     adjust size of characters in math mode    %%%%%% 
\newcommand{\proj}{{\mathds{P}}} 
\newcommand{\trans}{{\mathds{T}}} 
\newcommand{\mathsize}[2]{\mbox{\fontsize{#1}{2}\selectfont $#2$}}
\newcommand{\Proj}[1]{{\mathds{P}}_{\mathsize{7}{#1}}} 
\newcommand{\Trans}[1]{{\mathds{T}}_{\mathsize{7}{#1}}} 
\newcommand{\Rho}[1]{\rho_{\mathsize{7}{#1}}}
\newcommand{\Cas}[1]{C_{\mathsize{7}{#1}}}


%%  FIGURES AND PICTORIAL  EQUATIONS    %%

\def \drawqua (#1) {
\draw[postaction={decorate},decoration={markings,mark=at position #1 with {\large\arrow{>}}}] 
}
\def \drawanti (#1) {
\draw[postaction={decorate},decoration={markings,mark=at position #1 with {\large\arrow{<}}}] 
}

\newcommand{\tikeq}[1]{\vcenter{\hbox{\begin{tikzpicture}#1\end{tikzpicture}}}}
\newcommand{\tikeqbis}[1]{\hbox{\begin{tikzpicture}#1\end{tikzpicture}}}

%small matrices
\newenvironment{psmallmatrix}
{\left(\begin{smallmatrix}}
	{\end{smallmatrix}\right)}

% draw dashed lines 
\newcommand{\drawdash}{\draw[dash pattern=on 1pt off 1.3pt, line width=1.2]}

%%%%%%%%%%  FOOTNOTE ON PICTORIAL RULES %%%%%%%

%%%% counter-clock-wise quark loop with 3 external gluons  	 
\def \gggqloopCCW {\tikeqbis{\begin{scope}[scale=0.8,yshift=3mm]
\draw[anti] (0.2,0) arc(180:0:.3); \draw (0.2,0) arc(-180:0:.3); 
\draw[glu] (0.5,-0.6) -- (0.5,-0.3); \draw[glu] (-0.2,0) -- (0.2,0);  \draw[glu] (0.8,0) -- (1.2,0); 
\draw (-0.2,0) node[left] {$c$}; \draw (1.2,0) node[right] {$b$}; \draw (0.5,-0.6) node[below] {$a$}; 
\end{scope}}}

%%%% clock-wise quark loop with 3 external gluons  
\def \gggqloopCW  {\tikeqbis{\begin{scope}[scale=0.8,yshift=3mm]
\draw[qua] (0.2,0) arc(180:0:.3); \draw (0.2,0) arc(-180:0:.3); 
\draw[glu] (0.5,-0.6) -- (0.5,-0.3); \draw[glu] (-0.2,0) -- (0.2,0);  \draw[glu] (0.8,0) -- (1.2,0); 
\draw (-0.2,0) node[left] {$c$}; \draw (1.2,0) node[right] {$b$}; \draw (0.5,-0.6) node[below] {$a$}; 
\end{scope}}}


\def \qEdge (#1) {
\tikeq{\begin{scope}[scale=#1]
   \draw (0,0) node[left] {$i$};
  \draw[qua](0,0) -- (.8,0);
  \draw (.8,0) node[right] {$j$};
\end{scope}}}

\def \gEdge (#1) {
\tikeq{\begin{scope}[scale=#1]
   \draw (0,0) node[left] {$a$};
  \draw[glu](0,0) -- (.8,0);
  \draw (.8,0) node[right] {$b$};
\end{scope}}}

\def \gqqVert (#1) {
\tikeq{\begin{scope}[scale=#1]
   \draw (0,0) node[left] {$i$};
  \draw[qua](0,0) -- (.4,0);
  \draw[qua](.4,0) -- (.8,0);
  \draw (.8,0) node[right] {$j$};
  \draw[glu](.4,-0.4) -- (.4,0);
  \draw (.4,-0.4) node[below] {$a$};
    \end{scope}}}
  
 \def \gqbarqbarVert (#1) {
\tikeq{\begin{scope}[scale=#1]  
   \draw (0,0) node[left] {$i$};
  \draw[anti](0,0) -- (.4,0);
  \draw[anti](.4,0) -- (.8,0);
  \draw (.8,0) node[right] {$j$};
  \draw[glu](.4,-0.4) -- (.4,0);
  \draw (.4,-0.4) node[below] {$a$};
   \end{scope}}}
   
\def \gggVert (#1) {
\tikeq{\begin{scope}[scale=#1]   
   \draw (0,0) node[left] {$c$};
  \draw[glu](0,0) -- (.4,0)node{$\scriptstyle\bullet$};
  \draw[glu](.4,0) -- (.8,0);
  \draw (.8,0) node[right] {$b$};
  \draw[glu](.4,-0.4) -- (.4,0);
  \draw (.4,-0.4) node[below] {$a$};
 \end{scope}}}
 
\def \starVert (#1) {
\tikeq{\begin{scope}[scale=#1]  
   \draw (0,0) node[left] {$c$};
  \draw[glu](0,0) -- (.45,0);
  \draw[glu](.45,0) -- (.9,0);
  \draw (.9,0) node[right] {$b$};
  \draw (0.4,0) node {$\bigstar$};
  \draw[glu](.4,-0.4) -- (.4,-.05);
  \draw (.4,-0.4) node[below] {$a$};
\end{scope}}}
%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%  PROJECTORS %%%%%%%%%%%%%%%%

\def \Pqqbar (#1,#2) {
\tikeqbis{\begin{scope}[scale=#2]
	\coordinate (A) at (1.,0); 
	\coordinate (O) at (0,0); 
	\draw[anti] ($(A)+(0,-.3)$) -- ++ (.4,0) ;
	\draw[qua] ($(A)+(0,+.3)$) -- ++ (.4,0) ;
	\draw[anti] ($(A)+(1.,-.3)$) -- ++ (.4,0) ;
  \draw[qua] ($(A)+(1.,+.3)$) -- ++ (.4,0) ;
  \fill[white,draw=black] ($(O)+(1.7,.0)$) circle (.42);  
  \draw ($(O)+(1.7,0)$) node {$#1$};
  \end{scope}
}}
%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Pgg (#1,#2) {
\tikeqbis{\begin{scope}[scale=#2]
	\coordinate (A) at (1.,0); 
	\coordinate (O) at (0,0); 
	\draw[glu] ($(A)+(0,-.3)$) -- ++ (.4,0) ;
	\draw[glu] ($(A)+(0,+.3)$) -- ++ (.4,0) ;
	\draw[glu] ($(A)+(1.,-.3)$) -- ++ (.4,0) ;
  \draw[glu] ($(A)+(1.,+.3)$) -- ++ (.4,0) ;
  \fill[white,draw=black] ($(O)+(1.7,.0)$) circle (.42);  
  \draw ($(O)+(1.7,0)$) node {$#1$};
    \end{scope}}}
%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Pqqbaranti (#1,#2)  {
\tikeqbis{\begin{scope}[scale=#2]
	\coordinate (A) at (1.,0); 
	\coordinate (O) at (0,0); 
	\draw[anti] ($(A)+(0,-.25)$) -- ++ (.4,0) ;
	\draw[qua] ($(A)+(0,+.25)$) -- ++ (.4,0) ;
	\draw[qua] ($(A)+(.72,-.25)$) -- ++ (.4,0) ;
  \draw[anti] ($(A)+(.72,+.25)$) -- ++ (.4,0) ;
  \fill[white,draw=black] ($(O)+(1.55,.0)$) circle (.3);  
  \draw ($(O)+(1.55,0)$) node {$#1$};
 \end{scope}}}
 %%%%%%%%%%%%%%%%%%%%%%%%%
\def \Pqqbaranticross (#1,#2)  {
\tikeqbis{\begin{scope}[scale=#2]
	\coordinate (A) at (1.,0); 
	\coordinate (O) at (0,0); 
	\draw[anti] ($(A)+(0,-.25)$) -- ++ (.4,0) ;
	\draw[qua] ($(A)+(0,+.25)$) -- ++ (.4,0) ;
	\draw[anti] ($(A)+(.72,-.25)$) -- ++ (.4,0) ;
  \draw[qua] ($(A)+(.72,+.25)$) -- ++ (.4,0) ;
  \fill[white,draw=black] ($(O)+(1.55,.0)$) circle (.3);  
  \draw ($(O)+(1.55,0)$) node {$#1$};
  \draw ($(A)+(1.12,+.25)$) -- ++(0.4,-.5);
	\draw ($(A)+(1.12,-.25)$) -- ++(0.4,0.5);
  \draw[anti] ($(A)+(1.52,+.25)$) -- ++(0.35,-.0);
  \draw[qua] ($(A)+(1.52,-.25)$) -- ++(0.35,0.0);
 \end{scope}}}
%%%%%%%%%%%%%%%%%%%%%%
\def \Pthreebarqq  {\frac{1}{2} \left[ \ 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.7,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.7,0);
}
-
\tikeq{
		\coordinate (O) at (0,0);
		\draw (O) -- ++(0.7,.5);
		\draw ($(O)+(0,.5)$) -- ++(0.7,-0.5);
		\draw[qua] (O) -- ++(0.35,.25);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.35,-0.25);
} \ \right] }
%%%%%%%%%%%%%%%%%%%%%%
\def \Psixqq  {\frac{1}{2} \left[ \ 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.7,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.7,0);
}
+
\tikeq{
		\coordinate (O) at (0,0);
		\draw (O) -- ++(0.7,.5);
		\draw ($(O)+(0,.5)$) -- ++(0.7,-0.5);
		\draw[qua] (O) -- ++(0.35,.25);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.35,-0.25);
} \ \right]}
%%%%%%%%%%%%%%%%%%%%%%
\def \Poneqqbar { \displaystyle \frac1{\Nc} \
\tikeq{
    \coordinate (O) at (0,0);
    \draw[anti] (O) -- ++(0.1,0) -- ++(0,.5) -- ++(-0.1,0);  
    \draw[qua] ($(O)+(.5,0)$) -- ++(-0.1,0) -- ++(0,.5) -- ++(0.1,0);
}}
%%%%%%%%%%%%%%%%%%%%%%
\def \Peightqqbar {2 \ 
\tikeq{
        \coordinate (O) at (0,0);
        \draw[qua] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[anti] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[qua] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[anti] ($(O)+(1,.25)$) -- ++(.3,-.25);
}} 
%%%%%%%%%%%%%%%%%%%%%
\def \Pthreeqg  { \displaystyle \frac{1}{\CF} \, 
\tikeq{
		\coordinate (A) at (.3,.0);
		\coordinate (B) at (.7,.0);
    \draw[qua] ($(A)-(.3,-.35)$) -- (A);
    \draw[qua] (A) -- (B);
    \draw[qua] (B) -- ($(B)+(.3,.35)$) ;
    \draw[glu] ($(A)-(.3,.35)$) -- (A);
    \draw[glu] (B) -- ($(B)+(.3,-.35)$) ;
} }
%%%%%%%%%%%%%%%%%%%%%
\def \Psixqg  { \displaystyle \frac12 \ 
\tikeq{
		\coordinate (A) at (.3,.0);
		\coordinate (B) at (1.,.0);
    \draw[qua] ($(A)-(.3,-.25)$) -- ++(.7,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.7,0);
} 
-\frac{\Nc+1}2 \mathsize{11}{\Proj{\bm{3}} }
+ 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[glu] (A) -- ++(0.5,-.1);
		\draw[qua] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[qua] (B) -- ++(0.5,.1);
		\draw[glu] (A) --(B);
}}
%%%%%%%%%%%%%%%%%%%%%%
\def \Pfifteenqg  { \displaystyle \frac12 \ 
\tikeq{
		\coordinate (A) at (.3,.0);
		\coordinate (B) at (1.,.0);
    \draw[qua] ($(A)-(.3,-.25)$) -- ++(.7,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.7,0);
} 
+\frac{\Nc-1}2 \mathsize{11}{\Proj{\bm{3}} }
-
\tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[glu] (A) -- ++(0.5,-.1);
		\draw[qua] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[qua] (B) -- ++(0.5,.1);
		\draw[glu] (A) --(B);
}}
%%%%%%%%%%%%%%%%%%%%%%%
\def \Ponegg  { \displaystyle \frac1{\Nc^2-1} \ 
\tikeq{
		\coordinate (A) at (.0,.0);
		\coordinate (B) at (1,-.4);  
     \draw[glu] (A) .. controls +(0.5,0) and +(0.5,0) .. ($(A)+(0,-.4)$) ;            	
     \draw[glu] (B) .. controls +(-0.5,0) and +(-0.5,0) .. ($(B)+(0,.4)$); 
} 
}
%%%%%%%%%%%%%%%%%%%%%%
\def \PeightAgg  { \displaystyle \frac1{\Nc} \ 
\tikeq{
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[glu] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[glu] ($(O)+(1,.25)$) -- ++(.3,-.25);
}
}
%%%%%%%%%%%%%%%%%%%%%%
\def \PeightSgg  { \displaystyle \frac{\Nc}{\Nc^2-4} \ 
\tikeq{
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[glu] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[glu] ($(O)+(1,.25)$) -- ++(.3,-.25);
        \node [star, fill=black, star points=5, star point ratio=3.2, scale=.3] at ($(O)+(.3,.25)$) {};
        \node [star, fill=black, star points=5, star point ratio=3.2, scale=.3] at ($(O)+(1.,.25)$) {};
} 
}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ptengg}{ \displaystyle \frac12 \left[ \ 
\tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  -
\tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,-.5);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,.5);
} \ \right]
- \mathsize{11}{\Proj{\bm{8}_{\rm a}}}
}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ptwentysevengg}{ \displaystyle 
\bigg( 
\frac12 \ \tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  + 2\
\tikeq{
		\coordinate (A) at (0,.25);
		\coordinate (B) at (0,-.25);
		\coordinate (C) at (.5,.25);
		\coordinate (D) at (.5,-.25);
    \draw[glu] ($(A)-(.3,.0)$) -- (A);
    \draw[glu] ($(B)-(.3,.0)$) -- (B);
    \draw[glu] (C) -- ($(C)+(.3,.0)$);
    \draw[glu] (D) -- ($(D)+(.3,.0)$);
    \draw[qua] (A) -- (C);
    \draw[qua] (B) -- (D);
    \draw (A) -- (D);
    \draw (B) -- (C);
}  
\bigg) \bigg( \frac12 \left[ \ 
\tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  +
\tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,-.5);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,.5);
} \ \right] 
- \mathsize{11}{\Proj{\bm{8_{\rm s}}}}
- \mathsize{11}{\Proj{\bm{1}}}
\bigg)
}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Pzerogg}{ \displaystyle 
\bigg( 
\frac12 \ \tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  - 2\
\tikeq{
		\coordinate (A) at (0,.25);
		\coordinate (B) at (0,-.25);
		\coordinate (C) at (.5,.25);
		\coordinate (D) at (.5,-.25);
    \draw[glu] ($(A)-(.3,.0)$) -- (A);
    \draw[glu] ($(B)-(.3,.0)$) -- (B);
    \draw[glu] (C) -- ($(C)+(.3,.0)$);
    \draw[glu] (D) -- ($(D)+(.3,.0)$);
    \draw[qua] (A) -- (C);
    \draw[qua] (B) -- (D);
    \draw (A) -- (D);
    \draw (B) -- (C);
}  
\bigg) \bigg( \frac12 \left[ \ 
\tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  +
\tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,-.5);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,.5);
} \ \right] 
- \mathsize{11}{\Proj{\bm{8_{\rm s}}}}
- \mathsize{11}{\Proj{\bm{1}}}
\bigg)
}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ptwentysevenggcut}{ \displaystyle 
\bigg( 
\frac12 \ \tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  + 2\
\tikeq{
		\coordinate (A) at (0,.25);
		\coordinate (B) at (0,-.25);
		\coordinate (C) at (.5,.25);
		\coordinate (D) at (.5,-.25);
    \draw[glu] ($(A)-(.3,.0)$) -- (A);
    \draw[glu] ($(B)-(.3,.0)$) -- (B);
    \draw[glu] (C) -- ($(C)+(.3,.0)$);
    \draw[glu] (D) -- ($(D)+(.3,.0)$);
    \draw[qua] (A) -- (C);
    \draw[qua] (B) -- (D);
    \draw (A) -- (D);
    \draw (B) -- (C);
}  
\bigg)
}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Pzeroggcut}{ \displaystyle 
\bigg( 
\frac12 \ \tikeq{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
}  - 2\
\tikeq{
		\coordinate (A) at (0,.25);
		\coordinate (B) at (0,-.25);
		\coordinate (C) at (.5,.25);
		\coordinate (D) at (.5,-.25);
    \draw[glu] ($(A)-(.3,.0)$) -- (A);
    \draw[glu] ($(B)-(.3,.0)$) -- (B);
    \draw[glu] (C) -- ($(C)+(.3,.0)$);
    \draw[glu] (D) -- ($(D)+(.3,.0)$);
    \draw[qua] (A) -- (C);
    \draw[qua] (B) -- (D);
    \draw (A) -- (D);
    \draw (B) -- (C);
}  
\bigg)
}
%%%%%%%%%%%%%%%%%%%%%%
\def \Q {\displaystyle 
\frac12 \left[ \ 
\tikeq{\begin{scope}[scale=0.8] \coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);
\end{scope}}  +
\tikeq{\begin{scope}[scale=0.8] \coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,-.5);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,.5);
\end{scope}} \ \right] 
- \mathsize{11}{\Proj{\bm{8}_{\rm s}}}
- \mathsize{11}{\Proj{\bm{1}}}}
%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%   SOME TENSORS   %%%%%%%%%
\def \Igg {\tikeqbis{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,0);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,0);}}

\def \Xgg {\tikeqbis{
		\coordinate (A) at (.3,.0);
    \draw[glu] ($(A)-(.3,-.25)$) -- ++(.6,-.5);
    \draw[glu] ($(A)-(.3,.25)$) -- ++(.6,.5);}}
    
\def \Wm (#1) {\tikeqbis{\begin{scope}[scale=#1]
		\coordinate (A) at (0,.25);
		\coordinate (B) at (0,-.25);
		\coordinate (C) at (.5,.25);
		\coordinate (D) at (.5,-.25);
    \draw[glu] ($(A)-(.3,.0)$) -- (A);
    \draw[glu] ($(B)-(.3,.0)$) -- (B);
    \draw[glu] (C) -- ($(C)+(.3,.0)$);
    \draw[glu] (D) -- ($(D)+(.3,.0)$);
    \draw[qua] (A) -- (C);
    \draw[qua] (B) -- (D);
    \draw (A) -- (D);
    \draw (B) -- (C);\end{scope}}}
    
    \def \Wp (#1) {\tikeqbis{\begin{scope}[scale=#1]
		\coordinate (A) at (0,.25);
		\coordinate (B) at (0,-.25);
		\coordinate (C) at (.5,.25);
		\coordinate (D) at (.5,-.25);
    \draw[glu] ($(A)-(.3,.0)$) -- (A);
    \draw[glu] ($(B)-(.3,.0)$) -- (B);
    \draw[glu] (C) -- ($(C)+(.3,.0)$);
    \draw[glu] (D) -- ($(D)+(.3,.0)$);
    \draw[anti] (A) -- (C);
    \draw[anti] (B) -- (D);
    \draw (A) -- (D);
    \draw (B) -- (C);\end{scope}}}

%%%%%%%%%%  TRANSITION OPERATORS  %%%%%%%%%%%%%%%%

\def \Tonegg {
\tikeq{
		\coordinate (A) at (.0,.0);
		\coordinate (B) at (1,-.4);   
     \draw[glu] (A) .. controls +(0.5,0) and +(0.5,0) .. ($(A)+(0,-.4)$) ;            	
     \draw[qua] (B) .. controls +(-0.5,0) and +(-0.5,0) .. ($(B)+(0,.4)$); 
} }
%%%%%%%%%%%%%%%%%%%%%%
\def \TeightAgg  {
\tikeq{
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[qua] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[anti] ($(O)+(1,.25)$) -- ++(.3,-.25);
}}
%%%%%%%%%%%%%%%%%%%%%%
\def \TeightSgg  {
\tikeq{
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[qua] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[anti] ($(O)+(1,.25)$) -- ++(.3,-.25);
        \node [star, fill=black, star points=5, star point ratio=3.2, scale=.3] at ($(O)+(.3,.25)$) {};
      } }
%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%  AMPLITUDES  %%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%
\def \Mqoneqtwo {\tikeq{
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[qua] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
}}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\qqtchannel}[1]{\tikeq{\begin{scope}[scale=#1]
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[qua] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
\end{scope}
}}

\newcommand{\qquchannel}[1]{\tikeq{\begin{scope}[scale=#1]
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw (A) -- ++(0.4,0.5);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw(B) -- ++(0.4,-.5);
		\draw[glu] (A) --(B);
\end{scope}
}}


\def \Mqoneqone {\mathcal{B}_t \ \tikeq{
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[qua] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
} 
+ \mathcal{B}_u \  \tikeq{
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw (A) -- ++(0.4,0.5);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw(B) -- ++(0.4,-.5);
		\draw[glu] (A) --(B);
}}
%%%%%%%%%%%%%%%%%%%%%%
\def \Mqoneqtwobar {\tikeq{
		\coordinate (O) at (0,0);
		\draw[anti] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[anti] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
}}
%%%%%%%%%%%%%%%%%%%%%%
\def \Mqoneqonebar  {\tikeq{
        \coordinate (O) at (0,0);
        \draw[qua] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[anti] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[qua] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[anti] ($(O)+(1,.25)$) -- ++(.3,-.25);
}}
%%%%%%%%%%%%%%%%%%%%%%
\def \Mqoneqonebarbis { \mathcal{E}_s \ \tikeq{
        \coordinate (O) at (0,0);
        \draw[qua] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[anti] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.7,0);
        \draw[qua] ($(O)+(1,.25)$) -- ++(.3,.25);
        \draw[anti] ($(O)+(1,.25)$) -- ++(.3,-.25);
}+ \mathcal{E}_t \ \tikeq{
		\coordinate (O) at (0,0);
		\draw[anti] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[anti] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
}} 
%%%%%%%%%%%%%%%%%%%%%%
\def \Mqg { \tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[glu] (A) -- ++(0.5,-.1);
		\draw[qua] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[qua] (B) -- ++(0.5,.1);
		\draw[glu] (A) --(B);
}
 - \xi \ 
 \tikeq{
		\coordinate (A) at (.3,.0);
		\coordinate (B) at (.7,.0);
    \draw[qua] ($(A)-(.3,-.35)$) -- (A);
    \draw[qua] (A) -- (B);
    \draw[qua] (B) -- ($(B)+(.3,.35)$) ;
    \draw[glu] ($(A)-(.3,.35)$) -- (A);
    \draw[glu] (B) -- ($(B)+(.3,-.35)$) ;
}}
%%%%%%%%%%%%%%%%%%%%%%

\def \Mgggg { 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[glu] (A) -- ++(0.5,-.1);
		\draw[glu] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[glu] (B) -- ++(0.5,.1);
		\draw[glu] (A) --(B);
}
 - \xi \ 
\tikeq{
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.5,0);
        \draw[glu] ($(O)+(.8,.25)$) -- ++(.3,.25);
        \draw[glu] ($(O)+(.8,.25)$) -- ++(.3,-.25);
}
} 
%%%%%%%%%%%%%%%%%%%%%%

\def \Mggggbis { 
 \xibar  \ \tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1)coordinate(A);
		\draw[glu] (A) -- ++(0.5,-.1) ;
		\draw[glu] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[glu] (B) -- ++(0.5,.1);
		\draw[glu] (A) --(B);
}
 + \xi \ 
 \tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[glu] (A) -- ++(0.5,+0.6);
		\draw[glu] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[glu] (B) -- ++(0.5,-0.6);
		\draw[glu] (A) --(B);
}
} 
%%%%%%%%%%%%%%%%%%%%%%

\def \Mggqq { 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[anti] (A) -- ++(0.5,-.1);
		\draw[glu] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[qua] (B) -- ++(0.5,.1);
		\draw[qua] (A) --(B);
}
 - \xi \ 
\tikeq{
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.5,0);
        \draw[qua] ($(O)+(.8,.25)$) -- ++(.3,.25);
        \draw[anti] ($(O)+(.8,.25)$) -- ++(.3,-.25);
}
} 

%%%%%%%%%    OTHER BIRDTRACKS      %%%%%%%%%%%%%%%%%%


\def \xibird (#1,#2) {\tikeqbis{\begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (S) at   ($(O)+(.5,0)$); 
	        \coordinate (A2) at  ($(O)+(0,.5)$) ;  
	        \coordinate (A1) at  ($(A2)+(0,.6)$) ; 
	        \coordinate (A3) at  ($(A2)+(1.,0)$); 
	        \coordinate (A4) at  ($(A1)+(1.,0)$);  
	        \coordinate (B2) at  ($(O)-(0,.5)$) ;  
	        \coordinate (B1) at  ($(B2)-(0,.6)$) ;  
	        \coordinate (B3) at  ($(B2)+(1.,0)$);  
	        \coordinate (B4) at  ($(B1)+(1.,0)$);          
	        \drawdash  (A1) -- ++ (-1,0) arc (90:180:.3) -- ++ (0,-1.6) arc (-180:-90:.3) -- (B1);
	        \drawdash  (A2) -- ++ (-.7,0) arc (90:180:.2) -- ++ (0,-0.6) arc (-180:-90:.2) -- (B2);
	        \drawdash  (A4) -- ++ (1,0) arc (90:0:.3) -- ++ (0,-1.6) arc (0:-90:.3) -- (B4);
	        \drawdash  (A3) -- ++ (.7,0) arc (90:0:.2) -- ++ (0,-0.6) arc (0:-90:.2) -- (B3);
  \fill[color=gray!30!white,opacity=1] ($(A1)+(0,.1)$) rectangle ($(A3)+(0,-.1)$);  
  \draw ($(A1)+(.5,-.3)$) node {$\scriptstyle{{\cal M}}$};
  \fill[color=gray!30!white,opacity=1] ($(B2)+(0,.1)$) rectangle ($(B4)+(0,-.1)$); 
  \draw ($(B2)+(.5,-.3)$) node {$\scriptstyle{{\cal M}^*}$};
 \draw[glu] ($(A1)+(-0.6,0)$) -- ++ (0,.2) arc (180:90:.3) -- ++ (1.6,0) arc (90:0:.3) -- ++ (0,#2); 
\end{scope}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \xibirdstraight (#1,#2) {
\tikeqbis{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (S) at   ($(O)+(.5,0)$); 
	        \coordinate (A2) at  ($(O)+(0,.5)$) ;  
	        \coordinate (A1) at  ($(A2)+(0,.6)$) ; 
	        \coordinate (A3) at  ($(A2)+(1.,0)$); 
	        \coordinate (A4) at  ($(A1)+(1.,0)$);  
	        \coordinate (B2) at  ($(O)-(0,.5)$) ;  
	        \coordinate (B1) at  ($(B2)-(0,.6)$) ;  
	        \coordinate (B3) at  ($(B2)+(1.,0)$);  
	        \coordinate (B4) at  ($(B1)+(1.,0)$);          
    \draw ($(A1)+(-.2,.15)$) node {$1$};
    \draw ($(A2)+(-.2,-.15)$) node {$2$};
    \draw ($(A3)+(.2,-.15)$) node {$3$};
    \draw ($(A4)+(.2,.15)$) node {$4$};
	           
	        \draw[red]  (A1) -- ++ (-1,0) arc (90:180:.3) -- ++ (0,-1.6) arc (-180:-90:.3) -- (B1);
	        \draw[blue]  (A2) -- ++ (-.7,0) arc (90:180:.2) -- ++ (0,-0.6) arc (-180:-90:.2) -- (B2);
	        \draw[green]  (A4) -- ++ (1,0) arc (90:0:.3) -- ++ (0,-1.6) arc (0:-90:.3) -- (B4);
	        \draw[brown]  (A3) -- ++ (.7,0) arc (90:0:.2) -- ++ (0,-0.6) arc (0:-90:.2) -- (B3);

  \fill[color=gray!30!white,opacity=1] ($(A1)+(0,.1)$) rectangle ($(A3)+(0,-.1)$);  
  \draw ($(A1)+(.5,-.3)$) node {${\cal M}$};
  \fill[color=gray!30!white,opacity=1] ($(B2)+(0,.1)$) rectangle ($(B4)+(0,-.1)$); 
  \draw ($(B2)+(.5,-.3)$) node {${\cal M}^*$};
 
 \draw[glu] ($(O)+(-1.3,0)$) -- ($(O)+(#2,0)$) ; 
  \end{scope}
 }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \xibirdalpha (#1,#2,#3,#4) {
\tikeqbis{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (S) at   ($(O)+(.5,0)$); 
	        \coordinate (A2) at  ($(O)+(0,.5)$) ;  
	        \coordinate (A1) at  ($(A2)+(0,.6)$) ; 
	        \coordinate (A3) at  ($(A2)+(1.,0)$); 
	        \coordinate (A4) at  ($(A1)+(1.,0)$);  
	        \coordinate (B2) at  ($(O)-(0,.5)$) ;  
	        \coordinate (B1) at  ($(B2)-(0,.6)$) ;  
	        \coordinate (B3) at  ($(B2)+(1.,0)$);  
	        \coordinate (B4) at  ($(B1)+(1.,0)$);          	           
	        \draw[red]   ($(A1)+(.4,0)$) -- (A1) -- ++ (-1,0) arc (90:180:.3) -- ++ (0,-1.6) arc (-180:-90:.3) -- ($(B1)+(.2,0)$) ;
	        \draw[blue]   ($(A2)+(.4,0)$) -- (A2) -- ++ (-.7,0) arc (90:180:.2) -- ++ (0,-0.6) arc (-180:-90:.2) -- ($(B2)+(.2,0)$) ;
	        \draw[green]   ($(A4)+(-.4,0)$) -- (A4) -- ++ (1,0) arc (90:0:.3) -- ++ (0,-1.6) arc (0:-90:.3) -- ($(B4)+(-.2,0)$);
	        \draw[brown]   ($(A3)+(-.4,0)$) -- (A3) -- ++ (.7,0) arc (90:0:.2) -- ++ (0,-0.6) arc (0:-90:.2) -- ($(B3)+(-.2,0)$);
  \fill[white,draw=black] ($(A1)+(.5,-.3)$) circle (.42);   
  \draw ($(A1)+(.5,-.3)$) node {$#3$};
  \fill[white,draw=black] ($(B2)+(.5,-.3)$) circle (.42);  
  \draw ($(B2)+(.5,-.3)$) node {$#4$};
 \draw[glu] ($(A1)+(-0.6,0)$) -- ++ (0,.2) arc (180:90:.3) -- ++ (1.6,0) arc (90:0:.3) -- ++ (0,#2); 
  \end{scope}
 }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \xibirdalphastraight (#1,#2,#3,#4) {
\tikeqbis{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0);
	        \coordinate (A2) at  ($(O)+(0,.5)$) ;  
	        \coordinate (A1) at  ($(A2)+(0,.6)$) ; 
	        \coordinate (A3) at  ($(A2)+(1.,0)$); 
	        \coordinate (A4) at  ($(A1)+(1.,0)$);  
	        \coordinate (B2) at  ($(O)-(0,.5)$) ;  
	        \coordinate (B1) at  ($(B2)-(0,.6)$) ;  
	        \coordinate (B3) at  ($(B2)+(1.,0)$);  
	        \coordinate (B4) at  ($(B1)+(1.,0)$);          
    \draw ($(A1)+(-.2,.15)$) node {$1$};
    \draw ($(A2)+(-.2,-.15)$) node {$2$};
    \draw ($(A3)+(.2,-.15)$) node {$3$};
    \draw ($(A4)+(.2,.15)$) node {$4$};       
	        \draw[red]  ($(A1)+(.4,0)$) -- (A1) -- ++ (-1.,0) arc (90:180:.3) -- ++ (0,-1.6) arc (-180:-90:.3) -- ($(B1)+(.2,0)$) ;
	        \draw[blue]  ($(A2)+(.4,0)$) -- (A2) -- ++ (-.7,0) arc (90:180:.2) -- ++ (0,-0.6) arc (-180:-90:.2) -- ($(B2)+(.2,0)$);
	        \draw[green]  ($(A4)+(-.4,0)$) -- (A4) -- ++ (1,0) arc (90:0:.3) -- ++ (0,-1.6) arc (0:-90:.3) -- ($(B4)+(-.2,0)$);
	        \draw[brown] ($(A3)+(-.4,0)$) -- (A3) -- ++ (.7,0) arc (90:0:.2) -- ++ (0,-0.6) arc (0:-90:.2) -- ($(B3)+(-.2,0)$);
   \fill[white,draw=black] ($(O)+(.5,.8)$) circle (.42);  
  \draw ($(O)+(.5,.8)$) node {$#3$};
    \fill[white,draw=black] ($(O)+(.5,-.8)$) circle (.42);  
  \draw ($(O)+(.5,-.8)$) node {$#4$};
 \draw[glu] ($(O)+(-1.3,0)$) -- ($(O)+(#2,0)$) ; 
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Msquaredbird (#1) {
\tikeqbis{ \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (S) at   ($(O)+(.5,0)$); 
	        \coordinate (A2) at  ($(O)+(0,.5)$) ;  
	        \coordinate (A1) at  ($(A2)+(0,.6)$) ; 
	        \coordinate (A3) at  ($(A2)+(1.,0)$); 
	        \coordinate (A4) at  ($(A1)+(1.,0)$);  
	        \coordinate (B2) at  ($(O)-(0,.5)$) ;  
	        \coordinate (B1) at  ($(B2)-(0,.6)$) ;  
	        \coordinate (B3) at  ($(B2)+(1.,0)$);  
	        \coordinate (B4) at  ($(B1)+(1.,0)$);          
	        \drawdash  (A1) -- ++ (-1,0) arc (90:180:.3) -- ++ (0,-1.6) arc (-180:-90:.3) -- (B1);
	        \drawdash  (A2) -- ++ (-.7,0) arc (90:180:.2) -- ++ (0,-0.6) arc (-180:-90:.2) -- (B2);
	        \drawdash  (A4) -- ++ (1,0) arc (90:0:.3) -- ++ (0,-1.6) arc (0:-90:.3) -- (B4);
	        \drawdash  (A3) -- ++ (.7,0) arc (90:0:.2) -- ++ (0,-0.6) arc (0:-90:.2) -- (B3);
  \fill[color=gray!30!white,opacity=1] ($(A1)+(0,.1)$) rectangle ($(A3)+(0,-.1)$);  
  \draw ($(A1)+(.5,-.3)$) node {$\scriptstyle{{\cal M}}$};
  \fill[color=gray!30!white,opacity=1] ($(B2)+(0,.1)$) rectangle ($(B4)+(0,-.1)$); 
  \draw ($(B2)+(.5,-.3)$) node {$\scriptstyle{{\cal M}^*}$};
 \end{scope}}}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Operatorbird (#1) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at  ($(O)+(-.6,0)$) ;  
	        \coordinate (A1) at  ($(A2)+(-.6,0)$) ; 
	        \coordinate (A3) at  ($(A2)+(0,1)$); 
	        \coordinate (A4) at  ($(A1)+(0,1)$);  
	        \coordinate (B2) at  ($(O)-(-.6,0)$) ;  
	        \coordinate (B1) at  ($(B2)-(-.6,0)$) ;  
	        \coordinate (B3) at  ($(B2)+(0,1)$);  
	        \coordinate (B4) at  ($(B1)+(0,1)$);                
	        \drawdash  ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (180:270:.3) -- ++ (1.8,0) arc (-90:0:.3) -- ($(B1)+(0,.2)$) ;
	        \drawdash  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.8,0.) arc (-90:-0:.2) -- ($(B2)+(0,.2)$);
	        \drawdash  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (180:90:.3) -- ++ (1.8,0) arc (90:0:.3) -- ($(B4)+(0,-.2)$);
	        \drawdash ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.8,0) arc (90:0:.2) -- ($(B3)+(0,-.2)$);
  \fill[color=gray!30!white,opacity=1] ($(A2)+(.2,.1)$) rectangle ($(A4)+(-.2,-.1)$);  
  \draw ($(A1)+(.3,.5)$) node {$\scriptstyle{{\cal M}}$};
  \fill[color=gray!30!white,opacity=1] ($(B2)+(-.2,.1)$) rectangle ($(B4)+(.2,-.1)$);  
  \fill[color=white] ($(-.2,-1)$) rectangle ($(.2,2)$);  
  \draw[pattern=north west lines, pattern color=black] ($(-.2,-1)$) rectangle ($(.2,2)$);  
  \draw ($(B1)+(-.3,.5)$) node {$\scriptstyle{{\cal M}^*}$};
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Mtwototwo}[5] {
\tikeqbis{ \begin{scope}[scale=#5]
	        \coordinate (A2) at  (0,-0.3);  
	        \coordinate (A1) at  (0,0.3) ; 
	        \coordinate (A3) at  (1.,-0.3); 
	        \coordinate (A4) at  (1.,0.3);           
    \draw ($(A1)+(-0.6,.2)$) node {$#1$};
    \draw ($(A2)+(-0.6,-.2)$) node {$#2$};
    \draw ($(A3)+(0.6,-.2)$) node {$#4$};
    \draw ($(A3)+(1.1,0.)$) node {$\xi, \bm K$}; 
    \draw ($(A4)+(0.6,.2)$) node {$#3$}; 
    \draw ($(A4)+(1.2,0.)$) node {$\xibar, - \bm K$};      
	        \drawdash  (A1) -- ++ (-.7,0);
	        \drawdash (A2) -- ++ (-.7,0);
 		\drawdash  (A4) -- ++ (.7,0);
		\drawdash  (A3) -- ++ (.7,0);
  \fill[color=gray!30!white,opacity=1] ($(A1)+(0,.1)$) rectangle ($(A3)+(0,-.1)$);  
  \draw ($(A1)+(.5,-.3)$) node {${\cal M}$};
 \end{scope}}}


%%%%%%%%%%   KETS and BRAS  %%%%%%%%%%% 

\def \IdentitySinglet (#1,#2) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A) at  ($(O)+(0,-1.1)$) ;  
	        \coordinate (B) at  ($(O)+(0,-.7)$) ; 
	        \coordinate (C) at  ($(O)+(0,.7)$); 
	        \coordinate (D) at  ($(O)+(0,1.1)$);              
	        \drawdash  (A) -- ++ (#2,0);
	        \drawdash (B) -- ++ (#2,0);
	        \drawdash (C) -- ++ (#2,0);
	        \drawdash (D) -- ++ (#2,0);
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \OrthoKet (#1,#2) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at (.5,-.3) ;  
	        \coordinate (A1) at (1.1,-.3) ; 
	        \coordinate (A3) at (.5,.3) ;  
	        \coordinate (A4) at  (1.1,.3) ;   
    \draw (-0.15,-1.1) node {$\mathsize{8}{\bar{1}}$};
    \draw (-0.15,-0.6) node {$\mathsize{8}{\bar{2}}$};
    \draw (-0.15,0.7) node {$\mathsize{8}{4}$};
    \draw (-0.15,1.1) node {$\mathsize{8}{3}$};
	        \drawdash ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (360:270:.3) -- ++ (-0.8,0) ;
	        \drawdash  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (360:270:.2) -- ++ (-.3,0.) ;
	        \drawdash  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (0:90:.3) -- ++ (-0.8,0);
	        \drawdash ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (0:90:.2) -- ++ (-.3,0);
   \fill[white,draw=black] ($(O)+(.8,0)$) circle (.42);  
  \draw ($(O)+(.8,0)$) node {$#2$};
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \OrthoBra (#1,#2) {
\tikeq{  \begin{scope}[scale=#1]
 \coordinate (O) at (0,0); 
	        \coordinate (A2) at (-.5,-.3) ;  
	        \coordinate (A1) at (-1.1,-.3) ; 
	        \coordinate (A3) at (-.5,.3) ;  
	        \coordinate (A4) at  (-1.1,.3) ;  
    \draw (0.15,-1.1) node {$\mathsize{8}{\bar{1}}$};
    \draw (0.15,-0.6) node {$\mathsize{8}{\bar{2}}$};
    \draw (0.15,0.7) node {$\mathsize{8}{4}$};
    \draw (0.15,1.1) node {$\mathsize{8}{3}$}; 
	        \drawdash  ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (180:270:.3) -- ++ (0.8,0) ;
	        \drawdash  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.3,0.) ;
	        \drawdash  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (180:90:.3) -- ++ (0.8,0);
	        \drawdash ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.3,0);
   \fill[white,draw=black] ($(O)+(-.8,0)$) circle (.42);  
  \draw ($(O)+(-.8,0)$) node {$#2$};
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \OrthoBrau (#1,#2) {
\tikeq{  \begin{scope}[scale=#1]
 \coordinate (O) at (0,0); 
	        \coordinate (A2) at (-.5,-.3) ;  
	        \coordinate (A1) at (-1.1,-.3) ; 
	        \coordinate (A3) at (-.5,.3) ;  
	        \coordinate (A4) at  (-1.1,.3) ;  
    \draw (1.45,-1.1) node {$\mathsize{8}{\bar{1}}$};
    \draw (1.45,-0.6) node {$\mathsize{8}{\bar{2}}$};
    \draw (1.45,0.7) node {$\mathsize{8}{4}$};
    \draw (1.45,1.1) node {$\mathsize{8}{3}$}; 
          \drawdash  ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (180:270:.3) -- ++ (0.8,0) -- ++ (.7,0) -- ++ (.5,0);
          \drawdash  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.3,0.) 
          .. controls +(0.4,0) and +(-0.4,0) .. (0.8,0.7) 
          -- ++ (.4,0);
          \drawdash  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (180:90:.3) -- ++ (0.8,0) -- ++ (.7,0)-- ++ (.5,0);
          \drawdash ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.3,0) 
          .. controls +(0.4,0) and +(-0.4,0) .. (0.8,-0.7) 
          -- ++ (.4,0);
   \fill[white,draw=black] ($(O)+(-.8,0)$) circle (.42);  
  \draw ($(O)+(-.8,0)$) node {$#2$};
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \OrthoBrat (#1,#2) {
\tikeq{  \begin{scope}[scale=#1]
 \coordinate (O) at (0,0); 
	        \coordinate (A2) at (-.5,-.3) ;  
	        \coordinate (A1) at (-1.1,-.3) ; 
	        \coordinate (A3) at (-.5,.3) ;  
	        \coordinate (A4) at  (-1.1,.3) ;  
    \draw (1.45,-1.1) node {$\mathsize{8}{\bar{1}}$};
    \draw (1.45,-0.6) node {$\mathsize{8}{\bar{2}}$};
    \draw (1.45,0.7) node {$\mathsize{8}{4}$};
    \draw (1.45,1.1) node {$\mathsize{8}{3}$};   
          \drawdash  ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (180:270:.3) -- ++ (0.8,0) -- ++ (.7,0) -- ++ (.5,0);
          \drawdash  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.1,0.) 
          .. controls +(0.4,0) and +(-0.4,0) .. (0.8,1.1)  
          -- ++ (.4,0);
          \drawdash  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (180:90:.3) -- ++ (0.6,0) 
          .. controls +(0.4,0) and +(-0.4,0) .. (0.8,-0.7) 
          -- ++ (.4,0);
          \drawdash ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.3,0) -- ++ (.7,0) -- ++ (.5,0);
   \fill[white,draw=black] ($(O)+(-.8,0)$) circle (.42);  
  \draw ($(O)+(-.8,0)$) node {$#2$};
  \end{scope}
 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Balphabeta(#1,#2) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at  ($(O)+(-.5,0)$) ;  
	        \coordinate (A1) at  ($(A2)+(-.6,0)$) ; 
	        \coordinate (A3) at  ($(A2)+(0,1)$); 
	        \coordinate (A4) at  ($(A1)+(0,1)$);  
	        \coordinate (B2) at  ($(O)-(-.5,0)$) ;  
	        \coordinate (B1) at  ($(B2)-(-.6,0)$) ;  
	        \coordinate (B3) at  ($(B2)+(0,1)$);  
	        \coordinate (B4) at  ($(B1)+(0,1)$);                
	        \drawdash  ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (180:270:.3) -- ++ (1.6,0) arc (-90:0:.3) -- ($(B1)+(0,.2)$) ;
	        \drawdash  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.6,0.) arc (-90:-0:.2) -- ($(B2)+(0,.2)$);
	        \drawdash  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (180:90:.3) -- ++ (1.6,0) arc (90:0:.3) -- ($(B4)+(0,-.2)$);
	        \drawdash ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.6,0) arc (90:0:.2) -- ($(B3)+(0,-.2)$);
   \fill[white,draw=black] ($(O)+(-.8,.5)$) circle (.42);  
  \draw ($(O)+(-.8,.5)$) node {$\al$};
    \fill[white,draw=black] ($(O)+(.8,.5)$) circle (.42);  
  \draw ($(O)+(.8,.5)$) node {$\beta$};
 \draw[glu] ($(O)+(0,-0.8)$) -- ($(O)+(0,#2)$) ; 
  \end{scope}
 }}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Bbarone (#1) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at  ($(O)+(-.5,0)$) ;  
	        \coordinate (A1) at  ($(A2)+(-.6,0)$) ; 
	        \coordinate (A3) at  ($(A2)+(0,1)$); 
	        \coordinate (A4) at  ($(A1)+(0,1)$);  
	        \coordinate (B2) at  ($(O)-(-.5,0)$) ;  
	        \coordinate (B1) at  ($(B2)-(-.6,0)$) ;  
	        \coordinate (B3) at  ($(B2)+(0,1)$);  
	        \coordinate (B4) at  ($(B1)+(0,1)$);                
	        \draw[blue]  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.6,0.) arc (-90:-0:.2) -- ($(B2)+(0,.2)$);
	           \draw[brown] ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.6,0) arc (90:0:.2) -- ($(B3)+(0,-.2)$);
	        \draw[qua]  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.2) arc (0:90:.2) -- ++ (-.2,0) arc (90:180:.2) -- ++ (0,-1.4) arc (180:270:.2)  -- ++ (.2,0) arc (-90:0:.2) -- ($(A1)+(0,.2)$);
	         \draw[anti]  ($(B4)+(0,-.2)$) -- (B4) -- ++ (0,.2) arc (180:90:.2) -- ++ (.2,0) arc (90:0:.2) -- ++ (0,-1.4) arc (0:-90:.2)  -- ++ (-.2,0) arc (-90:-180:.2) -- ($(B1)+(0,.2)$);	        
   \fill[white,draw=black] ($(O)+(-.8,.5)$) circle (.42);  
  \draw ($(O)+(-.8,.5)$) node {$\al$};
    \fill[white,draw=black] ($(O)+(.8,.5)$) circle (.42);  
  \draw ($(O)+(.8,.5)$) node {$\beta$};
  \end{scope}
 }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Bbartwo (#1) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at  ($(O)+(-.5,0)$) ;  
	        \coordinate (A1) at  ($(A2)+(-.6,0)$) ; 
	        \coordinate (A3) at  ($(A2)+(0,1)$); 
	        \coordinate (A4) at  ($(A1)+(0,1)$);  
	        \coordinate (B2) at  ($(O)-(-.5,0)$) ;  
	        \coordinate (B1) at  ($(B2)-(-.6,0)$) ;  
	        \coordinate (B3) at  ($(B2)+(0,1)$);  
	        \coordinate (B4) at  ($(B1)+(0,1)$);               
	        \draw[anti]  ($(A1)+(0,.2)$) -- (A1) -- ++ (0,-.5) arc (180:270:.3) -- ++ (1.6,0) arc (-90:0:.3) -- ($(B1)+(0,.2)$) ;
	        \draw[blue]  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.6,0.) arc (-90:-0:.2) -- ($(B2)+(0,.2)$);
	        \draw[qua]  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.5) arc (180:90:.3) -- ++ (1.6,0) arc (90:0:.3) -- ($(B4)+(0,-.2)$);
	        \draw[brown] ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.6,0) arc (90:0:.2) -- ($(B3)+(0,-.2)$);
   \fill[white,draw=black] ($(O)+(-.8,.5)$) circle (.42);  
  \draw ($(O)+(-.8,.5)$) node {$\al$};
    \fill[white,draw=black] ($(O)+(.8,.5)$) circle (.42);  
  \draw ($(O)+(.8,.5)$) node {$\beta$};
  \end{scope}
 }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \birdKtwo (#1) {
\tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at  ($(O)+(-.5,0)$) ;  
	        \coordinate (A1) at  ($(A2)+(-.6,0)$) ; 
	        \coordinate (A3) at  ($(A2)+(0,1)$); 
	        \coordinate (A4) at  ($(A1)+(0,1)$);               
	        \draw[blue]  ($(A2)+(0,.2)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.3,0.);
	         \draw[brown] ($(A3)+(0,-.2)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.3,0) ;
	        \draw[qua]  ($(A4)+(0,-.2)$) -- (A4) -- ++ (0,.2) arc (0:90:.2) -- ++ (-.2,0) arc (90:180:.2) -- ++ (0,-1.4) arc (180:270:.2)  -- ++ (.2,0) arc (-90:0:.2) -- ($(A1)+(0,.2)$);              
   \fill[white,draw=black] ($(O)+(-.8,.5)$) circle (.42);  
  \draw ($(O)+(-.8,.5)$) node {$\al$};
  \end{scope}
 }
 = \frac{K_\al}{K_2} \ \ 
 \tikeq{  \begin{scope}[scale=#1]
	        \coordinate (O) at (0,0); 
	        \coordinate (A2) at  ($(O)+(-.5,0)$) ;  
	        \coordinate (A3) at  ($(A2)+(0,1)$);      
	        \draw[blue]  ($(A2)+(0,.5)$) -- (A2) -- ++ (0,-.2) arc (180:270:.2) -- ++ (.3,0.);
	         \draw[brown] ($(A3)+(0,-.5)$) -- (A3) -- ++ (0,.2) arc (180:90:.2) -- ++ (.3,0) ;
  \end{scope}
 }}


%%%%%%%%%%%%%%     FIERZ   %%%%%%%%%%%%%%%

\def \Fierzone {
\tikeq{
    \coordinate (O) at (0,0);
    \draw[anti] ($(O)+(0,0)$) -- ++(0.7,0);
    \draw[qua] ($(O)+(0,.7)$) -- ++(0.7,0);
}\
=\ \frac{1}{\Nc}\
\tikeq{
    \coordinate (O) at (0,0);
    \draw[anti] (O) -- ++(0.1,0) -- ++(0,.7) -- ++(-0.1,0);  
    \draw[qua] ($(O)+(.5,0)$) -- ++(-0.1,0) -- ++(0,.7) -- ++(0.1,0);
}
+ 2\ 
\tikeq{
        \coordinate (O) at (0,0);
        \draw[qua] ($(O)+(0,.7)$) -- ++(.3,-.35);
        \draw[anti] (O) -- ++(.3,.35);
        \draw[glu] ($(O)+(.3,.35)$) -- ++(.7,0);
        \draw[qua] ($(O)+(1,.35)$) -- ++(.3,.35);
        \draw[anti] ($(O)+(1,.35)$) -- ++(.3,-.35);
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Fierztwo {
2 \ \tikeq{
		\coordinate (O) at (0,0);
		\draw[anti] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[anti] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.7)$) -- ++(0.4,0) coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
}\
= \ 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[anti] (O) -- ++(0.1,0) -- ++(0,.7) -- ++(-0.1,0);  
		\draw[qua] ($(O)+(.5,0)$) -- ++(-0.1,0) -- ++(0,.7) -- ++(0.1,0);
}
- \frac{1}{\Nc}\ 
\tikeq{
		\coordinate (O) at (0,0);
		\draw[anti] ($(O)+(0,0)$) -- ++(0.7,0);
		\draw[qua] ($(O)+(0,.7)$) -- ++(0.7,0);
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def \Fierzthree {
2 \ \tikeq{
		\coordinate (O) at (0,0);
		\draw[qua] ($(O)+(0,0)$) -- ++(0.4,0) coordinate(A);
		\draw[qua] (A) -- ++(0.4,0);
		\draw[qua] ($(O)+(0,.5)$) -- ++(0.4,0)coordinate(B);
		\draw[qua] (B) -- ++(0.4,0);
		\draw[glu] (A) --(B);
} 
\ = \ - \ 
\tikeq{		
		\drawqua(0.25) (0,0) -- (0.7,0.5);  
		\drawqua(0.25) (0,0.5) -- (0.7,0);
}
\ + \ \frac{1}{\Nc}\ 
\tikeq{
		\drawqua(0.5) (0,0) -- (0.7,0);  
		\drawqua(0.5) (0,0.5) -- (0.7,0.5);	
}}


%%%%%%%%%%%%   APPENDIX  B  %%%%%%%%%%%%
\newcommand{\vacuum}[2]{\tikeqbis{\begin{scope}[scale=#2]
  \draw[qua] (-0.5,0.4) -- (0,0.4); \draw[qua] (0,0.4) -- (0.5,0.4); 
  \draw[anti] (-0.5,-0.4) -- (0,-0.4); \draw[anti] (0,-0.4) -- (0.5,-0.4); 
  \draw (-0.5,0.4) -- (-0.5,-0.4);  \draw (0.5,0.4) -- (0.5,-0.4);
 \draw (0,0) node {$\times$};
 \draw[glu][red] (0,-0.4) -- (0,0.4) ;
 \draw (-0.2,0.2) node {$#1$}; 
 \draw[dashed] (-.8,0) -- (.8,0);
 \end{scope}
 }}
 
\newcommand{\medium}[1]{\tikeqbis{\begin{scope}[scale=#1]
  \fill[color=blue!30!white,opacity=0.5] ($(-.4,-.6)$) rectangle (.4,.6);  
  \drawqua(0.3) (-0.8,0.4) -- (0,0.4); \drawqua(0.8) (0,0.4) -- (0.8,0.4); 
  \drawanti(0.3) (-0.8,-0.4) -- (0,-0.4); \drawanti(0.8) (0,-0.4) -- (0.8,-0.4); 
  \draw (-0.8,0.4) -- (-0.8,-0.4);  \draw (0.8,0.4) -- (0.8,-0.4);
 \draw (0,0) node {$\times$};
 \draw[glu][red] (0,-0.4) -- (0,0.4) ;
  \draw (-0.2,0.2) node {$\bm{\scriptstyle{q}}$}; 
 \draw[dashed] (-1.2,0) -- (1.2,0);
 \end{scope}
 }}


\newcommand{\Cnkq}[2]{\tikeqbis{\begin{scope}[scale=#2]
  \fill[color=blue!30!white,opacity=0.5] (-1.3,-0.8) rectangle (1.4,1.2); 
  \drawqua(0.12) (-2,0.5) -- (0,0.5); \drawqua(0.9) (0,0.5) -- (2,0.5); 
  \drawanti(0.12) (-2,-0.5) -- (0,-0.5); \drawanti(0.9) (0,-0.5) -- (2,-0.5); 
  \draw (-2,0.5) -- (-2,-0.5);  \draw (2,0.5) -- (2,-0.5);
 \draw 
 (-1.,0) node{$\times$} 
 (-0.5,0) node {$\times$} 
 (0,0) node {$\times$} 
 (1.,0) node {$\times$} 
 (1.8,1.1) node {$\bm{\scriptstyle{k}}$}  (0.3,0.3) node {$\bm{\scriptstyle{q}}$} (-1.2,0.3) node {$\bm{\scriptstyle{\ell_1}}$} (-0.2,0.3) node {$\bm{\scriptstyle{\ell_i}}$} ; 
  \draw[glu] (-1,-0.5) -- (-1,0.5) ;
  \draw[glu] (-0.3,0.9) -- (-0.5,0); \draw[glu] (-0.5,0) -- (-0.7,0.5) ;
  \draw[glu] (0,-0.5) -- (0,0.9);
 \draw[glu][red] (0.5,-0.5) -- (0.5,0.5) ;
  \draw[glu] (0.85,-0.5) -- (1,0); \draw[glu] (1,0) -- (1.15,-0.5);
\draw[glu] (-1.6,.5) arc (180:90:.4) -- (2,0.9)  arc (90:0:.4) -- (2.4,-0.5)
arc (0:-180:.4); 
\draw[fill=white,opacity=#1] (1.6,-0.5) circle (0.1); 
\draw[dashed] (-2.2,0) -- (2.6,0);
\end{scope}
}}


\newcommand{\Cnbisellipse}[1]{\tikeqbis{\begin{scope}[scale=#1]
  \fill[color=blue!30!white,opacity=0.5] (-1.2,-0.8) rectangle (1.3,1.2); 
  \drawqua(0.12) (-2,0.5) -- (0,0.5); \drawqua(0.92) (0,0.5) -- (2.1,0.5); 
  \drawanti(0.12) (-2,-0.5) -- (0,-0.5); \drawanti(0.92) (0,-0.5) -- (2.1,-0.5); 
  \draw (-2,0.5) -- (-2,-0.5);  \draw (2.1,0.5) -- (2.1,-0.5);
 \draw 
 (-1.,0) node{$\times$}  (-0.5,0) node {$\times$} (0,0) node {$\times$} (0.5,0) node {$\times$} 
 (1.,0) node {$\times$} 
 (1.8,1.1) node {$\bm{\scriptstyle{k}}$}  (1.6,0.3) node {$\bm{\scriptstyle{K}}$}
 (1.6,0.63) node {$\bm{\scriptstyle{-K}}$} 
 (-0.75,-0.25) node {$\bm{\scriptstyle{\ell_1}}$}
 (-0.2,-0.25) node {$\bm{\scriptstyle{\ell_i}}$} 
 (0.3,-0.25) node {$\bm{\scriptstyle{\kappa}}$}  ; 
  \draw[glu] (-1,-0.5) -- (-1,0.5) ;
  \draw[glu] (-0.3,0.9) -- (-0.5,0); \draw[glu] (-0.5,0) -- (-0.7,0.3) ;
  \draw[glu] (0,-0.5) -- (0,0.9);
  \draw[glu][red] (1.5,-0.5) arc (180:90:.2) arc (-90:0:.2) 
-- (1.9,0.1) arc (0:90:.2) -- (-1,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-1.5,0.5) ; 
 \draw[glu] (0.5,-0.5) -- (0.5,0.3) ;
 \draw[glu] (0.85,-0.5) -- (1,0); \draw[glu] (1,0) -- (1.15,-0.5);
\draw[glu] (-1.6,.5) arc (180:90:.4) -- (2,0.9)  arc (90:0:.4) -- (2.4,-0.5)
arc (0:-180:.35); 
\draw[fill=white,opacity=1] (1.7,-0.15) .. controls +(-0.1,0) and +(-0.1,0) .. (1.7,-0.65); 
\draw[fill=white,opacity=1] (1.7,-0.15) .. controls +(0.1,0) and +(0.1,0) .. (1.7,-0.65);
 \draw[dashed] (-2.2,0) -- (2.7,0);
\end{scope}
}}

\newcommand{\GammanKK}[1]{\tikeqbis{\begin{scope}[scale=#1]
  \fill[color=blue!30!white,opacity=0.5] (-1.2,-0.8) rectangle (1.3,1.2); 
  \drawqua(0.12) (-2,0.5) -- (0,0.5); \drawqua(0.92) (0,0.5) -- (2.1,0.5); 
  \drawanti(0.12) (-2,-0.5) -- (0,-0.5); \drawanti(0.92) (0,-0.5) -- (2.1,-0.5); 
  \draw (-2,0.5) -- (-2,-0.5);  \draw (2.1,0.5) -- (2.1,-0.5);
 \draw 
 (-1.,0) node{$\times$}  (-0.5,0) node {$\times$}  (0,0) node {$\times$} (0.5,0) node {$\times$} 
 (1.,0) node {$\times$} (2,1.1) node {$\bm{\scriptstyle{k}}$} (1.6,0.3) node {$\bm{\scriptstyle{K}}$}
 (1.6,0.63) node {$\bm{\scriptstyle{-K}}$} 
 (-0.75,-0.25) node {$\bm{\scriptstyle{\ell_1}}$}
 (-0.2,-0.25) node {$\bm{\scriptstyle{\ell_i}}$} 
 (0.3,-0.25) node {$\bm{\scriptstyle{\kappa}}$}  ; 
  \draw[glu] (-1,-0.5) -- (-1,0.5) ;
  \draw[glu] (-0.3,0.9) -- (-0.5,0); \draw[glu] (-0.5,0) -- (-0.7,0.3) ;
  \draw[glu] (0,-0.5) -- (0,0.9);
  \draw[glu][red] (1.5,-0.5) arc (180:90:.2) arc (-90:0:.2) 
-- (1.9,0.1) arc (0:90:.2) -- (-1,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-1.5,0.5) ; 
 \draw[glu] (0.5,-0.5) -- (0.5,0.3) ;
 \draw[glu] (0.85,-0.5) -- (1,0); \draw[glu] (1,0) -- (1.15,-0.5);
\draw[glu] (-1.6,.5) arc (180:90:.4) -- (2,0.9)  arc (90:0:.4) -- (2.4,-0.5)
arc (0:-180:.35) -- (1.7,-0.3)  ; 
\draw[fill=white,opacity=1] (1.7,-0.3) circle (0.1); 
\draw[dashed] (-2.2,0) -- (2.7,0);
\end{scope}
}}


\newcommand{\GammazeroNorescatt}[2]{\tikeqbis{\begin{scope}[scale=#2]
 \drawqua(0.3) (-0.8,0.4) -- (0,0.4); \drawqua(0.8) (0,0.4) -- (0.8,0.4); 
  \drawanti(0.3) (-0.8,-0.4) -- (0,-0.4); \drawanti(0.8) (0,-0.4) -- (0.8,-0.4); 
  \draw (-0.8,0.4) -- (-0.8,-0.4);  \draw (0.8,0.4) -- (0.8,-0.4);
 \draw (0,0) node {$\times$};
 \draw  (0.6,1) node {$\bm{\scriptstyle{k}}$};
 \draw[glu][red] (0,-0.4) -- (0,0.4) ;
  \draw[glu] (-0.4,0.4) arc (180:90:.4) -- (0.8,0.8) arc  (90:0:.4) -- (1.2,-0.4) 
  arc  (0:-180:.4) ; 
 \draw[fill=white,opacity=1] (0.4,-0.4) circle (0.1); 
 \draw[fill=white,opacity=#1] (-0.4,0.4) circle (0.1); 
 \draw[dashed] (-1,0) -- (1.4,0);
 \end{scope}
}}


\newcommand{\blueblob}[1]{\tikeqbis{\begin{scope}[scale=#1,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
  \draw[anti] ($(A)-(0.5,0)$) -- ($(A)-(.2,0)$); 
  \draw[anti] ($(A)+(.2,0)$) -- ($(A)+(0.5,0)$);
  \draw[qua] ($(B)-(0.5,0)$) -- ($(B)-(.2,0)$); 
  \draw[qua] ($(B)+(.2,0)$) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$) ;
  \draw ($(C)+(0.4,0.2)$) node {$\bm{\scriptstyle{k}}$} ;
  \fill[color=blue!15!white,opacity=1] ($(A)-(.2,.15)$) rectangle ($(C)+(.2,.2)$);
 \end{scope}
}}


\newcommand{\rescatta}[3]{\tikeq{\begin{scope}[scale=#3,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
  \drawanti(0.35) ($(A)-(0.5,0)$) -- (A); \draw (A) -- ($(A)+(0.5,0)$);
  \drawqua(0.35) ($(B)-(0.5,0)$) -- (B); \draw (B) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$);
  \draw ($(C)+(-0.5,0.17)$) node {$#1$} ;
  \draw ($(C)+(0.4,0.2)$) node {$#2$} ;
  \draw[glu]  (A) -- (C);
  \draw[color=blue] (O) node {$\times$};
 \end{scope}
}}
  
  
\newcommand{\rescattb}[3]{\tikeq{\begin{scope}[scale=#3,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
 \drawanti(0.35) ($(A)-(0.5,0)$) -- (A); \draw (A) -- ($(A)+(0.5,0)$);
  \drawqua(0.35) ($(B)-(0.5,0)$) -- (B); \draw (B) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$);
  \draw ($(C)+(-0.5,0.17)$) node {$#1$} ;
  \draw ($(C)+(0.4,0.2)$) node {$#2$} ;
  \draw[glu]  ($(C)+(-0.2,0)$) -- (O) ; \draw[glu] (O) --  ($(B)+(0.2,0)$); 
  \draw[color=blue] (O) node {$\times$};
 \end{scope}
}}
  
  \newcommand{\rescattc}[3]{\tikeq{\begin{scope}[scale=#3,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
  \drawanti(0.35) ($(A)-(0.5,0)$) -- (A); \draw (A) -- ($(A)+(0.5,0)$);
  \drawqua(0.35) ($(B)-(0.5,0)$) -- (B); \draw (B) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$);
  \draw ($(C)+(-0.5,0.2)$) node {$#1$} ;
  \draw ($(C)+(0.4,0.2)$) node {$#2$} ;
  \draw[glu]  ($(C)+(-0.2,0)$) -- (O) ;  \draw[glu]  (O) --  ($(C)+(0.2,0)$); 
  \draw[color=blue] (O) node {$\times$};
 \end{scope}
}}

\newcommand{\rescattd}[3]{\tikeq{\begin{scope}[scale=#3,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
  \drawanti(0.35) ($(A)-(0.5,0)$) -- (A); \draw (A) -- ($(A)+(0.5,0)$);
  \drawqua(0.35) ($(B)-(0.5,0)$) -- (B); \draw (B) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$);
  \draw ($(C)+(-0.5,0.2)$) node {$#1$} ;
  \draw ($(C)+(0.4,0.2)$) node {$#2$} ;
  \draw[glu]  ($(A)+(-0.2,0)$) -- (O) ; \draw[glu] (O) --  ($(A)+(0.2,0)$); 
  \draw[color=blue] (O) node {$\times$};
 \end{scope}
}}

\newcommand{\rescatte}[3]{\tikeq{\begin{scope}[scale=#3,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
  \drawanti(0.35) ($(A)-(0.5,0)$) -- (A); \draw (A) -- ($(A)+(0.5,0)$);
  \drawqua(0.35) ($(B)-(0.5,0)$) -- (B); \draw (B) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$);
  \draw ($(C)+(-0.5,0.2)$) node {$#1$} ;
  \draw ($(C)+(0.4,0.2)$) node {$#2$} ;
  \draw[glu]  ($(B)+(-0.2,0)$) -- (O);  \draw[glu]  (O) --  ($(B)+(0.2,0)$); 
  \draw[color=blue] (O) node {$\times$};
 \end{scope}
}}
  
  
\newcommand{\rescattf}[3]{\tikeq{\begin{scope}[scale=#3,yshift=-5]
  \coordinate (O) at (0,0);
  \coordinate (A) at ($(O)+(0,-0.3)$);
  \coordinate (B) at ($(O)+(0,0.3)$); 
  \coordinate (C) at ($(O)+(0,0.6)$); 
  \drawanti(0.35) ($(A)-(0.5,0)$) -- (A); \draw (A) -- ($(A)+(0.5,0)$);
  \drawqua(0.35) ($(B)-(0.5,0)$) -- (B); \draw (B) -- ($(B)+(0.5,0)$);
  \draw[glu] ($(C)-(0.5,0)$) -- ($(C)+(0.5,0)$);
  \draw ($(C)+(-0.5,0.2)$) node {$#1$} ;
  \draw ($(C)+(0.4,0.2)$) node {$#2$} ;
  \draw[glu]  ($(A)$) -- (O) --  ($(B)$); 
  \draw[color=blue] (O) node {$\times$};
 \end{scope}
}}


\newcommand{\HardRescatta}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
\drawqua(0.12) (-0.5,0.5) -- (1.5,0.5); 
\draw[glu](0.5,0.3) -- (0.5,0) ; \draw[glu](0.5,0) -- (0.5,-0.3) ;
\draw (0.5,0) node {$\times$};
\drawanti(0.1) (-0.5,-0.5) -- (1.5,-0.5); 
\draw[glu][red] (-0.1,-0.5) .. controls +(0.2,0.2) and +(-0.3,0) .. (0.5,-0.3) -- (1.1,-0.3) arc (-90:0:.2) 
-- (1.3,0.1) arc (0:90:.2) -- (1.1,0.3) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-0.1,0.5) ; 
\draw  (-0.5,0.5) --  (-0.5,-0.5);  \draw  (1.5,0.5) --  (1.5,-0.5); 
\draw[dashed] (-0.7,0) -- (1.7,0);
 \end{scope}
}}

\newcommand{\HardRescattb}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
\drawqua(0.12) (-0.5,0.5) -- (1.5,0.5); 
\draw[glu](0.5,0.5) -- (0.5,0) ; \draw[glu](0.5,0) -- (0.5,-0.5) ;
\draw (0.5,0) node {$\times$};
\drawanti(0.1) (-0.5,-0.5) -- (1.5,-0.5); 
\draw[glu][red] (-0.1,-0.5) .. controls +(0.2,0.2) and +(-0.3,0) .. (0.5,-0.3) -- (1.1,-0.3) arc (-90:0:.2) 
-- (1.3,0.1) arc (0:90:.2) -- (1.1,0.3) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-0.1,0.5) ; 
\draw  (-0.5,0.5) --  (-0.5,-0.5);  \draw  (1.5,0.5) --  (1.5,-0.5); 
\draw[dashed] (-0.7,0) -- (1.7,0);
 \end{scope}
}}


\newcommand{\HardRescattc}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
\drawqua(0.12) (-0.5,0.5) -- (1.5,0.5); 
\draw[glu] (0.3,0.5) -- (0.3,0) ; \draw[glu](0.3,0) -- (0.3,-0.5) ;
\draw (0.3,0) node {$\times$};
\drawanti(0.1) (-0.5,-0.5) -- (1.5,-0.5); 
\draw[glu][red] (0.6,-0.5) arc (180:90:.2) -- (1.1,-0.3) arc (-90:0:.2) 
-- (1.3,0.1) arc (0:90:.2) -- (1.1,0.3) -- (0.8,0.3) arc (-90:-180:.2) ; 
\draw  (-0.5,0.5) --  (-0.5,-0.5);  \draw  (1.5,0.5) -- (1.5,-0.5); 
\draw[dashed] (-0.7,0) -- (1.7,0);
 \end{scope}
}}

\newcommand{\HardRescattd}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
\drawqua(0.12) (-0.5,0.5) -- (1.5,0.5); 
\draw[glu](0.5,0.3) -- (0.5,0) ; \draw[glu](0.5,0) -- (0.5,-0.5) ;
\draw (0.5,0) node {$\times$};
\drawanti(0.1) (-0.5,-0.5) -- (1.5,-0.5); 
\draw[glu][red] (-0.1,-0.5) .. controls +(0.2,0.2) and +(-0.3,0) .. (0.5,-0.3) -- (1.1,-0.3) arc (-90:0:.2) 
-- (1.3,0.1) arc (0:90:.2) -- (1.1,0.3) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-0.1,0.5) ; 
\draw  (-0.5,0.5) --  (-0.5,-0.5);  \draw  (1.5,0.5) --  (1.5,-0.5); 
\draw[dashed] (-0.7,0) -- (1.7,0);
 \end{scope}
}}


\newcommand{\HardRescatte}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
\drawqua(0.12) (-0.5,0.5) -- (1.5,0.5); 
\draw[glu](0.5,0.5) -- (0.5,0) ; \draw[glu](0.5,0) -- (0.5,-0.5) ;
\draw (0.5,0) node {$\times$};
\drawanti(0.1) (-0.5,-0.5) -- (1.5,-0.5); 
\draw[glu][red] (0.8,-0.5) arc (180:90:.2) -- (1.1,-0.3) arc (-90:0:.2) 
-- (1.3,0.1) arc (0:90:.2) -- (1.1,0.3) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-0.1,0.5) ; 
\draw  (-0.5,0.5) --  (-0.5,-0.5);  \draw  (1.5,0.5) --  (1.5,-0.5); 
\draw[dashed] (-0.7,0) -- (1.7,0);
 \end{scope}
}}


\newcommand{\HardRescattf}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
\drawqua(0.12) (-0.5,0.5) -- (1.5,0.5); 
\draw[glu](0.5,0.3) -- (0.5,0) ; \draw[glu](0.5,0) -- (0.5,-0.5) ;
\draw (0.5,0) node {$\times$};
\drawanti(0.1) (-0.5,-0.5) -- (1.5,-0.5); 
\draw[glu][red] (0.8,-0.5) arc (180:90:.2) -- (1.1,-0.3) arc (-90:0:.2) 
-- (1.3,0.1) arc (0:90:.2) -- (1.1,0.3) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (-0.1,0.5) ; 
\draw  (-0.5,0.5) --  (-0.5,-0.5);  \draw  (1.5,0.5) --  (1.5,-0.5); 
\draw[dashed] (-0.7,0) -- (1.7,0);
\draw (0.16,-0.25) node {$\bm{\scriptstyle{\kappa}}$} (0.35,-0.25) node {$\uparrow$} ; 
 \end{scope}
}}


\newcommand{\Gammazerobis}[1]{\tikeqbis{\begin{scope}[scale=#1]
  \drawqua(0.2) (-1,0.5) -- (0,0.5); \drawqua(0.9) (0,0.5) -- (2.1,0.5); 
  \drawanti(0.2) (-1,-0.5) -- (0,-0.5); \drawanti(0.9) (0,-0.5) -- (2.1,-0.5); 
  \draw (-1,0.5) -- (-1,-0.5);  \draw (2.1,0.5) -- (2.1,-0.5);
 \draw (0.5,0) node {$\times$}; 
  \draw[glu][red] (1,-0.5) arc (180:90:.2) -- (1.7,-0.3) arc (-90:0:.2) 
-- (1.9,0.1) arc (0:90:.2) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (0,0.5) ; 
\draw[glu] (0.5,-0.5) -- (0.5,0.3) ;
\draw[glu] (-0.6,.5) arc (180:90:.4) -- (2,0.9)  arc (90:0:.4) -- (2.4,-0.5)
arc (0:-180:.35) -- (1.7,-0.3) ; 
 \draw[fill=white,opacity=1] (-0.6,0.5) circle (0.1); 
 \draw[fill=white,opacity=1] (1.7,-0.3) circle (0.1); 
 \draw[dashed] (-1.2,0) -- (2.65,0);
 \end{scope}
}}

\newcommand{\MMgluon}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
  \drawqua(0.2) (-1,0.5) -- (0,0.5); \drawqua(0.9) (0,0.5) -- (2.1,0.5); 
  \drawanti(0.2) (-1,-0.5) -- (0,-0.5); \drawanti(0.9) (0,-0.5) -- (2.1,-0.5); 
  \draw (-1,0.5) -- (-1,-0.5);  \draw (2.1,0.5) -- (2.1,-0.5);
 \draw  (0.5,0) node {$\times$}; 
  \draw[glu][red] (0.7,-0.5) arc (180:90:.2) -- (1.7,-0.3) arc (-90:0:.2) 
-- (1.9,0.1) arc (0:90:.2) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (0.2,0.5) ; 
\draw[glu] (0.5,-0.5) -- (0.5,0.3) ;
  \fill[color=gray!30!white,opacity=1] (0.1,-0.6) rectangle (0.9,-0.2); 
  \fill[color=gray!30!white,opacity=1] (0.1,0.2) rectangle (0.9,0.6);  
\draw (0.5,0.4) node {$\scriptstyle{{\cal M}}$}  ;
\draw (0.5,-0.4) node {$\scriptstyle{{\cal M}^*}$}  ;
\draw[glu] (-0.6,.5) arc (180:90:.4) -- (2,0.9)  arc (90:0:.4) -- (2.4,-0.5)
arc (0:-180:.35) -- (1.7,-0.3) ; 
 \draw[fill=white,opacity=1] (-0.6,0.5) circle (0.1); 
 \draw[fill=white,opacity=1] (1.7,-0.3) circle (0.1); 
 \draw[dashed] (-1.2,0) -- (2.6,0);
 \end{scope}
}}

\newcommand{\MMquark}[1]{\tikeq{\begin{scope}[scale=#1,yshift=-5]
  \drawqua(0.2) (-1,0.5) -- (0,0.5); \drawqua(0.9) (0,0.5) -- (2.1,0.5); 
  \drawanti(0.2) (-1,-0.5) -- (0,-0.5); \drawanti(0.9) (0,-0.5) -- (2.1,-0.5); 
  \draw (-1,0.5) -- (-1,-0.5);  \draw (2.1,0.5) -- (2.1,-0.5);
 \draw (0.5,0) node {$\times$} ; 
  \draw[glu][red] (0.7,-0.5) arc (180:90:.2) -- (1.7,-0.3) arc (-90:0:.2) 
-- (1.9,0.1) arc (0:90:.2) -- (0.5,0.3) .. controls +(-0.3,0) and +(0.2,-0.2) .. (0.2,0.5) ; 
\draw[glu] (0.5,-0.5) -- (0.5,0.3) ;
  \fill[color=gray!30!white,opacity=1] (0.1,-0.6) rectangle (0.9,-0.2); 
  \fill[color=gray!30!white,opacity=1] (0.1,0.2) rectangle (0.9,0.6);  
\draw (0.5,0.4) node {$\scriptstyle{{\cal M}}$}  ;
\draw (0.5,-0.4) node {$\scriptstyle{{\cal M}^*}$}  ;
\draw[glu] (-0.6,.5) arc (180:90:.4) -- (2,0.9)  arc (90:0:.4) -- (2.4,-0.5)
arc (0:-180:.35) ; 
 \draw[fill=white,opacity=1] (-0.6,0.5) circle (0.1); 
 \draw[fill=white,opacity=1] (1.7,-0.5) circle (0.1); 
 \draw[dashed] (-1.2,0) -- (2.6,0);
 \end{scope}
}}

\newcommand{\ggtoggschannel}[1]{\tikeq{\begin{scope}[scale=#1]
        \coordinate (O) at (0,0);
        \draw[glu] ($(O)+(0,.5)$) -- ++(.3,-.25);
        \draw[glu] (O) -- ++(.3,.25);
        \draw[glu] ($(O)+(.3,.25)$) -- ++(.5,0);
        \draw[glu] ($(O)+(.8,.25)$) -- ++(.3,.25);
        \draw[glu] ($(O)+(.8,.25)$) -- ++(.3,-.25);
 \end{scope}
}}

\newcommand{\ggtoggtchannel}[1]{\tikeq{\begin{scope}[scale=#1]
		\coordinate (O) at (0,0);
		\draw[glu] ($(O)+(0,0)$) -- ++(0.5,.1) coordinate(A);
		\draw[glu] (A) -- ++(0.5,-.1);
		\draw[glu] ($(O)+(0,.7)$) -- ++(0.5,-.1)coordinate(B);
		\draw[glu] (B) -- ++(0.5,.1);
		\draw[glu] (A) --(B);
\end{scope}
}}


